Energy Efficient SDN and SDR Joint Adaptation of CPU Utilization Based on Experimental Data Analytics

In this paper we propose a hybrid softwarized architecture of Network Function Virtualization (NFV) where Software-Defined Networking (SDN) and Software-Defined Radio (SDR) components are integrated to form a cloud-based communication system. We analyze CPU utilization and power consumption in the OpenIreland testbed for different parameter settings and use case scenarios of this NFV architecture. The experiment results show different behaviour between SDN data plane switching and SDR in terms of CPU utilization and parallelization, which provides insights for processing aggregation and power savings when integrating them together in a cloud-based system. We then propose a power saving scheme with flexible CPU allocation that can reduce the overall power consumption of the system. Our results show that our proposed NFV architecture and its power saving scheme can save up to 20% power consumption compared to conventional scheme where SDN and SDR are separately deployed.

==> sections/system_model.tex <==
\section{System Model}
\label{sec:system_model}

%In this section we first present our network architecture with \ac{SDN} and \ac{SDR} integrated approach. 

%Then we investigate the relationship between CPU utilisation and power consumption, the results of which provides an insight for the later power saving algorithm we implement.

%\subsection{Network Architecture}

We propose an \ac{MEC} as an example for a use case of \ac{SDN} and \ac{SDR} integrated architecture, as shown in Figure~\ref{fig:MEC_architecture}. This architecture can be for example adopted in systems for inter-vehicle communications \cite{1543745}.
The architecture is all software-defined and network functions are virtualized. As the two major network functions for this architecture, \ac{SDN} and \ac{SDR} functions are integrated in the edge servers (i.e. \ac{MEC} nodes). Vehicular networks are illustrated at end user side. Inside the \ac{MEC} nodes, SDN switches, eNodeB \acp{BBU}, 4G/5G core function, and computational resources for \ac{MEC} tasks utilize the same group of servers. In this paper, we focus on the integration of the communication part, i.e., \ac{SDN} and \ac{SDR} components.

%\textcolor{red}{..are you going to provide more details about this architecture? If not this section should probably merge with the next one.}
%\textcolor{blue}{in fact the MEC architecture is not important here. Instead, we put more details on an SDN-SDR integrated architecture, and merged with the next section}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/overall_architecture.png}
	\caption{proposed MEC architecture}
	\label{fig:MEC_architecture}
	\vspace{-0.1in}
\end{figure}



% \subsection{Power consumption vs CPU utilisation Experiments}

% To investigate the power consumption of the \ac{SDN} and \ac{SDR} integrated \ac{NFV} system, the first step we carry out is a measurement of the CPU power consumption  vs CPU utilisation rate. 
% %There are some papers providing power consumption general theoretical models~\cite{experiment_c4_Lin}-\cite{experiment_LIN2018940}. However, those general model didn't consider the difference between the difference CPU brands, which have proven to be one factor to the power consumption~\cite{experiment_LIN2018940}.
% %Even for one CPU, different working temperature also cause the CPU power consumption increase~\cite{experiment_Karel}.
% %Considering those difficult in using theoretical power consumption model, In our case, 
% We use testbed measurement and adopt \ac{NN} to get the regression model for the CPU utilisation rate vs. CPU power consumption in our testbed.

% Our CPU type is: $Intel$ $Core^{TM}$ $i7\-4810MQ$. We measure 70 data points (blue points in Fig. ~\ref{fig:NN_plot}) for Power consumption vs CPU load. To generate different level of CPU load we use a customised CPU load generator written by ourselves in Linux bash, and scale the CPU load from 0\% to 100\%.
% For measuring the Power consumption of the CPU we use the Linux application 'turbostat', which returns the CPU power consumption in watts.
% %\textcolor{red}{... how do you generate the data points?}\textcolor{blue}{we use scalable CPU process bash program built by ourselves. added in the text.}

% %Then at the inference phase, we can infer an power consumption through the input utilisation rate.
% %The \ac{NN} which is driven by data is a good tool in solving regression problems. 
% To build the regression curve (red curve in Fig. ~\ref{fig:NN_plot}),
% we build two-layer \ac{NN}, shown in Fig. \ref{fig:NN_structure}. This \ac{NN} includes two dense layers, with 20 nodes in each layer and uses 'relu' as activation function. The input of the \ac{NN} is the CPU's utilisation, the output is CPU's power consumption. The results in Fig.~\ref{fig:NN_plot} shows that the fitted curve presents a two-sector of linear shape with a knee point around 50\% CPU utilisation. This method can be used to get corresponding curves for other types of CPU as well. With the measurement and curve fittings, we observe the features of the power consumption for different CPU cores, which provides the insight for the power optimisation solutions proposed later in this paper.

% %\textcolor{red}{...you don't really say why this curve is important, what is its scope for the paper objectives?}\textcolor{blue}{We have added some statements to address the scope of the curve}

% \begin{figure}[h]
% 	\centering
% \includegraphics[width=0.45\textwidth]{figures/NN_structure.png}
% 	\caption{The structure of Neural Networks}
% 	\label{fig:NN_structure}
%     \vspace{-0.1in}
% \end{figure}



% \begin{figure}[h]
% 	\centering
% \includegraphics[width=0.45\textwidth]{figures/NN_plot.png}
% 	\caption{Regression curve for the CPU utilisation rate vs. CPU power consumption}
% 	\label{fig:NN_plot}
%     \vspace{-0.1in}
% \end{figure}


% \begin{table}[ht]
% \caption{Statistical analysis of the SNR for the downlink, at 55 dB transmitter gain.}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
%  \textbf{Distance} & \textbf{Average} & \textbf{Standard} & \textbf{Confidence} & \textbf{Max} & \textbf{Min} \\ 
%   \textbf{(cm)} &  \textbf{(dB)} & \textbf{Deviation (dB)} & \textbf{Interval (dB)} & \textbf{(dB)} & \textbf{(dB)} \\
%  \hline
%  0   & 31.1044 & 1.5805 & 0.0980  & 34.0   & 27.9 \\  
%  20  & 29.8855 & 1.1352 & 0.0704 & 32.2 & 27.2 \\ 
%  40  & 28.3759 & 0.7280  & 0.0451 & 29.9 & 26.8 \\ 
%  60  & 23.8751 & 1.0637 & 0.0659 & 25.3 & 14.7 \\ 
%  80  & 21.3312 & 1.0483 & 0.0650  & 23.1 & 16.4\\ 
%  100 & 16.6697 & 1.5552 & 0.0964 & 18.3 & 12.4 \\ 
%  120 & 14.8763 & 0.7983 & 0.0495 & 17.3 & 12.6 \\ 
%  140 & 13.1189 s& 0.9459 & 0.0586 & 15.5 & 9.0\\ 
%  160 & 12.2334 & 0.8596 & 0.0533 & 15.1 & 9.2 \\ 
%  180 & 13.2411 & 0.7260  & 0.0450  & 15.2 & 11.0 \\ 
%  200 & 11.6577 & 0.8913 & 0.0552 & 13.5 & 9.1 \\ 
%  220 & 11.3320  & 0.3551 & 0.0220  & 12.3 & 10.2 \\ 
%  240 & 6.0951  & 0.3073 & 0.0190  & 6.9  & 3.2\\
 
%  \hline
% \end{tabular}
% \label{table:3}
% \end{table}

% \subsection{Throughput measurements and mode selection}

% We also measure the maximum throughout using the same experimental setup shown in Fig.~\ref{fig:Results_Scenario} and Fig.~\ref{fig:measurement_setup}. 
% In the \ac{3GPP} \ac{LTE} standard, the throughput is determined by the \ac{MCS} index and number of \ac{PRBs} utilized for transmission. We allocate 25 \ac{PRBs} for both downlink and sidelink in our experiment. Therefore, at each measurement location we seek to reach the maximum throughput by increasing the \ac{MCS} index of the transmitters, for the downlink and sidelink, and record the maximum throughput while the observed \ac{BLER} remains at zero. The highest modulation for the downlink is 64 \ac{QAM} and the highest modulation for the sidelink is 16 \ac{QAM} according to the \ac{LTE} standard. Figs.~\ref{fig:Throughput_vs_Distance_40} and~\ref{fig:Throughput_vs_Distance_30} show how the throughput varies according to the position of the remote \ac{UE}; the trends follow closely those reported for the \ac{SNR}.

% %Fig.~\ref{fig:Throughput_vs_Distance_40} shows the throughput versus distance for both the sidelink (orange curve) and the downlink (blue curve), with the transmitter gain of the sidelink fixed at 40 dB. From Fig.~\ref{fig:Throughput_vs_Distance_40}, we can see that if the remote \ac{UE} is moved from eNodeB to the cell edge and beyond, the remote \ac{UE} should do downlink till it reaches around 160 cm, after which the throughput through sidelink relay gets better. Therefore at 160 cm the remote \ac{UE} should perform sidelink. After 256 cm, which is the cell edge, the downlink does not work, the remote \ac{UE} has to perform sidelink to get cellular coverage. 

% %Fig.~\ref{fig:Throughput_vs_Distance_30} shows the same result with the sidelink transmitter gain at 30 dB. We can see that around 180 cm is the switching point for remote \ac{UE}. We can also see that most of the time throughout for sidelink is low in comparison to throughput when the gain was 40 dB for sidelink. But the throughput is still higher in comparison to downlink, suggesting that remote \ac{UE} should switch to sidelink after 180 cm. 

% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/Throughput_vs_Distance_pic2}  %trim= l b r t
% 	\caption{Maximum throughput versus distance, for 40 dB sidelink gain.}
%     	\label{fig:Throughput_vs_Distance_40}
% \end{figure}

% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/Throughput_vs_Distance_pic1}  %trim= l b r t
% 	\caption{Maximum throughput versus distance for 30 dB sidelink gain.}
%     	\label{fig:Throughput_vs_Distance_30}
% \end{figure}







